(Amplified) Banded Matrix Factorization: A unified approach to private training

Matrix factorization (MF) mechanisms for differential privacy (DP) have substantially improved the state-of-the-art in privacy-utility-computation tradeoffs for ML applications in a variety of scenarios, but in both the centralized and federated settings there remain instances where either MF cannot be easily applied, or other algorithms provide better tradeoffs (typically, as $\epsilon$ becomes small). In this work, we show how MF can subsume prior state-of-the-art algorithms in both federated and centralized training settings, across all privacy budgets. The key technique throughout is the construction of MF mechanisms with banded matrices (lower-triangular matrices with at most $\hat{b}$ nonzero bands including the main diagonal). For cross-device federated learning (FL), this enables multiple-participations with a relaxed device participation schema compatible with practical FL infrastructure (as demonstrated by a production deployment). In the centralized setting, we prove that banded matrices enjoy the same privacy amplification results as the ubiquitous DP-SGD algorithm, but can provide strictly better performance in most scenarios -- this lets us always at least match DP-SGD, and often outperform it.

==> backups/abstract.tex <==
% Matrix factorization (MF) mechanisms for differential privacy (DP) have substantially improved the state-of-the-art in privacy/utility/computation tradeoffs for ML application over the ubiquitous DP-SGD algorithm in a variety of settings, including: 1) centralized training with $\epsilon > 2$ and a modest number of training steps (e.g., $\dimension \le 10^5$), and 2) cross-device federated learning where each device participates once in training. 

% In this work, we greatly expand the applicability of MF, showing that it can fully subsume DP-SGD. The key technique throughout is the construction of MF mechanisms with banded matrices. For cross-device federated learning, this enables multiple-participations with a relaxed device participation schema compatible with practical FL infrastructure. For centralized training, we give privacy amplification results for MF that are identical to the best known results for DP-SGD (corresponding to a diagonal matrix in MF), but can be strictly improved in most scenarios by amplifying a matrix with $\bands > 1$ bands.  Finally, for both domains using $\bands$-banded matrices substantially reduces the memory and time complexity of per-iteration noise generation from $\calO(\dimension)$, the total number of iterations, to $\calO(\bands)$ (a constant independent of $\dimension$).

==> backups/b-min-sep.tex <==
\rnote{I think much of this stuff would fit better in the introduction.}
\ctodo{I removed the banded fro mthe previous section, can we define it here? It's commented out below.}
% \paragraph{Banded matrices}
% We say a (general) matrix $\bfX$ is $\bands$-banded if for all $i,j \in [n]$, $|i -j| \ge \bands$ implies $\bfX\idx{i}{j} = 0$. While this is off-by-one from the typical definition of bandwidth ($\bfX$ has bandwidth $b-1$), our definition will be useful as it will be natural to match $\bands$-banded matrices with $\minsep$-min-separation. Further, for $\bands$-banded lower-triangular matrices (which will play a central role), $\bands$ intuitively gives the number of bands in the matrix.  

% We may want to move some of this to related work.
While \multiepoch-participation is a good fit for centralized training infrastructure, in cross-device federated learning the order in which data is processed cannot be tightly controlled, as devices make local decisions about if and when they will participate in training \citep{FLO,bonawitz2019towards}. This led to the development of alternative DP training protocols that could benefit from some amplification, such as that of \citet{balle2020privacy}. The cross-device FL setting was in fact a primary motivation for the development of the DP-FTRL algorithm \citep{kairouz2021practical}, which allows performance competitive with DP-SGD analyzed with amplification-via-sampling, but applies to arbitrary data processing patterns (with sensitivity calculated based on the minimum separation between participations).  \citet{denisov22matfact} improved on this approach in the single-participation setting by using matrix factorization in place of tree aggregation; the dense lower-triangular matrix mechanisms introduced in this work could be used in cross-device FL, but only if each client was restricted to participate at most once.  \citet{choquette22multiepoch} extended to \citet{denisov22matfact}, but focused on \multiepoch-participation, which as noted above is only feasible in centralized training scenarios. Hence the key open question we address here: \emph{Can matrix-factorization DP-FTRL (\MFFTRL) be extended to the cross-device federated learning setting with multiple client participations?} 

This question is of substantial practical importance, as \citet{choquette22multiepoch} showed \MFFTRL can substantially outperform tree-aggregation-based DP-FTRL. However, in practice the limitation to a single participation (single epoch) is prohibitive in many private training scenarios, as increasing the number of clients per round (equivalent to the batch size in centralized training) and hence the total epochs of training is perhaps the single most important technique in improving privacy/utility tradeoffs in differentially private machine learning \citep{ponomareva2023dpfy}.

It is also worth clarifying exactly what the extension of \MFFTRL to cross-device FL requires. An arbitrary factorization $\bfA = \bfB \bfC$ could be used under any participation schema (including \bparticipation). However, in order to make deploying such a mechanism useful, it is essential that we can tightly bound $\sensd(\bfC)$, and hence state tight privacy guarantees. Of course, even this is not enough: we could take the trivial factorization $\bfB \leftarrow \bfA$ and $\bfC \leftarrow \bfI$, and tightly bounding sensitivity would be trivial. Hence, we need to be able to both generate ``good'' factorizations (\btodo{Need to reference, possibly forward, a defintion of ``good''}) and bound their sensitivity. The best way to do this is to find a way to efficiently represent the constraint $\sensd(\bfC) \le 1$ in the mathematical program solved to find \emph{optimal} factorizations $\bfA = \bfB \bfC$.

Our approach to extending \MFFTRL to cross-device FL thus begins with a generalization of \multiepoch-participation, \bparticipation, which can practically be enforced by cross-device FL systems \btodo{Will need to say more about this somewhere.}  Then, we introduce a class of matrix mechanisms that perform extremely well while allowing for the efficient computation of sensitivity, and hence, efficient convex optimization to find the necessary matrix factorizations.

We define a participation schema where the distance between any two participations is \emph{at least} \minsep, rather than \emph{exactly} $\minsep$ as in \multiepoch-participation:
\begin{definition}\label{def:bparticipation}
The \textbf{\bparticipation} schema is given by
\[
  \Pi_b = \left\{\pi \subseteq [n]  \mid \{i, j\} \subseteq \pi, i \ne j \Rightarrow |i - j| \ge \minsep\right\}.
\]
\end{definition}


Note that for \multiepoch-participation, $|\Pi_{(\maxpart,\minsep)}| = \minsep$, a fact \citet[Eq. 3]{choquette22multiepoch} critically exploited when computing sensitivity as brute force computation of $\max_{\pi \in \Pi}$.  With \bparticipation, we have $|\Pi_b| = \calO(\exp(n))$,  \btodo{Could compute something more exact here.} and hence such brute force approaches will be impractical even when we require $\bfC\tp \bfC \ge 0$.

Fortunately, this challenge can be surmounted for $\bands$-banded $\bfC$. We begin with the following Corollary.

\begin{cor}\label{cor:matrix_to_vector_sens}
For any dimensionality $\mdim \ge 1$, when per-step contributions are bounded by $\clipnorm=1$, consider a participation schema $\Pi \subseteq \Pi_b$ and matrix $\bfC$ such that for all $\pi \in \Pi$, for any $i, j \in \pi$ with $i \ne j$, we have $\left<\bfC\idx{:}{i}, \bfC\idx{:}{j} \right> = 0$ (that is, any pair of columns of $\bfC$ corresponding to distinct iterations $i, j$ where the same example might participate must be orthogonal).  Then,
\[
\senss(\bfC) = \sensv(\bfC).
\]
\end{cor}
\begin{proof}
The orthogonality condition implies $\bfC\idx{:}{\pi}\tp \bfC\idx{:}{\pi}$ is a diagonal matrix, with the (non-negative) norms of the selected columns forming the diagonal, and hence Condition 2 of \citet[Thm. G.1]{choquette22multiepoch} applies to $\bfC\idx{:}{\pi}$, and the result follows.
\end{proof}

Observe that a sufficient condition for \cref{cor:matrix_to_vector_sens} to hold is that $\bfC$ is $\minsep$-banded.\footnote{A stronger version of \cref{cor:matrix_to_vector_sens} can of course be proved immediately, requiring only  $\left<\bfC\idx{:}{i}, \bfC\idx{:}{j} \right> \ge 0$. However, this extra generality is not necessary for our purposes.} In the following theorem, we present two practical approaches to bounding sensitivity:


\newcommand{\vals}{c}  % Values being optimized
% TODO - consider switching i and t in the code
% and here ... to be t is better as a "budget" and
% i is better as an index.
\newcommand{\bi}{i}  % Total number of elements to choose, including x(t)
\newcommand{\ridx}{t} % Rightmost index
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}


\begin{algorithm}[t]
\caption{Efficient sensitivity calculation for \bparticipation} \label{alg:minsepsens}
\begin{algorithmic}%[1]
\State \textbf{Inputs:} min-separation $\minsep$, Gram matrix $\bfX$, max participations $\maxpart$
\State Initialize $F \in \R^{n \times k}$
\For{$m = 1, \dots, k$}
\For{$i = n, \dots, 1$}
 \Comment{We use the convention that $F[s,t] = 0$ if $s,t$ are out-of-bounds.}
\State $F[i, m] = \max{\Big(\bfX_{ii} + F[i+b, m-1], F[i+1, m]\Big)}$
\EndFor
\EndFor
\Return $\sqrt{F[1, k]}$
\end{algorithmic}
\end{algorithm}

\newcommand{\indpi}{u(\pi)}

\begin{theorem}\label{thm:minsepsens}
Let $\bfC \in \R^\dimdim$ be a lower-triangular $\bands$-banded matrix, and and the \bparticipation schema $\Pi_b$.  Further, suppose $k'$ upper-bounds the actual maximum number of participations that occurred in a data stream $\obs$ (at worst, we may take $k' \le \ceil{\frac{n}{b}}$):
Then:
\begin{enumerate}
\item \cref{alg:minsepsens} computes $\senss(\bfC)$ under schema $\Pi_b$ in polynomial time, and if $k' < \ceil{\frac{n}{b}}$, may produce a tighter bound on sensitivity for streams matching the actual participations in $\obs$.\footnote{Recall that for our notion of adjacency, all adjacent streams $\obsp$ must have this property.}
\item If $\kappa$ is an upper-bound on the column norms of $\bfC$, that is $\ \forall j \in [n], \ \norm{\bfC\idx{:}{j}} \le \kappa$, then the sensitivity is bounded by $\kappa \sqrt{k'}$.
\end{enumerate}
\end{theorem}
%
\begin{proof}
For \cref{alg:minsepsens}, let $\vals \in \R^\dimension$ with entries $\vals_i = \norm{\bfC\idx{:}{i}}^2$ for $i \in \{0, \dots, \dimension-1\}$. We have
\begin{equation}\label{eq:orthcolnorm}
\senss(\bfC) 
  = \max_{\pi \in \Pi_b} \norm{\bfC \indpi} 
  = \max_{\pi \in \Pi_b} \norm{\sum_{i \in \pi} \bfC\idx{:}{i}}  
  = \max_{\pi \in \Pi_b} \sqrt{\sum_{i \in \pi} c_i}
\end{equation}
where $\indpi \in \{0, 1\}^\dimension$ is given by $\indpi_i = 1$ if $i \in \pi$ and $0$ otherwise. The last equality follows from the orthogonality condition on sufficiently separated columns of $\bfC$. It is straightforward to verify the dynamic program of \cref{alg:minsepsens} constructs a feasible $\pi$ which attains the maximum.
\end{proof}

We find that $\bfC$ matrices normalized to have equal column norms perform well, and so hence often the $\kappa \sqrt{\minsep}$ bound of \cref{thm:minsepsens} is tight, and can easily be incorporated into optimization (in fact, the constant scaling can be handled post-optimization, so it is sufficient to simply enforce a fixed maximum column norm).

==> backups/setting.tex <==
\section{Setting and notation}
\btodo{Work in progress}
\btodo{Decide whether we want to write ``example'', ``user'', or ``record'' for the general unit of privacy. We used ``example'' in the multi-epoch paper, so goiing with that for now.}
We build on the multi-epoch setting of \citet{choquette22multiepoch}, which we summarize here.  

Assume a database of $\numusers$ examples (users in FL, records in general DP applications) that is processed as a stream over $\dimension$ steps. A batch of $\batchsize$ examples is selected on each step $i$, and processed via an adaptively chosen function (e.g., computing a gradient at the current model), producing a vector of $\ell_2$ norm at most $\clipnorm$. These vectors are summed and provided to the DP mechanism as $\obs_i \in \R^\mdim$, which releases a privatized function of $[\obs_1, \dots, \obs_i]$, the stream so far. When a particular example contributes to the sum $\obs_i$, we say it \emph{participates} on step $i$. We are primarily interested in the case where $\numusers < \dimension \cdot \batchsize$, and hence each example is used on more than one step. This is the multiple epoch setting of ML.

\btodo{We probably need to also re-state the definition of adjacent streams. It might clarify things to introduce notation for individual examples, as well as a ``data processing function'' which assigns examples to batches for each iteration.}

\paragraph{Participation schemas}
A \emph{participation schema} $\Pi$ is a set of possible \emph{participation patterns} $\pi \in \Pi$, with each $\pi \subseteq [\dimension]$ indicating a set of steps in which any single example might participate. That is, if example $j$ participates in rounds $r_j \subseteq [n]$, then we require $r_j \subseteq \pi$ for some $\pi \in \Pi$.

Simple examples include \emph{single-participation} (each record contributes at most once, $\Pi = \big\{ \{1\}, \{2\}, \dots \{\dimension\}\big\}$) and \emph{every-step participation} (each record might contribue on every step, as in full gradient descent, $\Pi = \{ [\dimension]\}$).  \citet{choquette22multiepoch} studied \emph{fixed-epoch-order participation}, denoted \emph{\multiepoch-participation}, where each example participates at most $\maxpart$ times, with any adjacent participations exactly $\minsep$ steps apart: formally, $\Pi$ is the set of all $\pi$ such that $|\pi| \le \maxpart$, and if $\pi = \{i_1, \dots, i_k\}$ indexed in increasing order, we have $\forall j \in \{2, \dots, k\}, i_j - i_{j-1} = \minsep$. For example $\maxpartsep{3}{2}$-participation has $\Pi = \{\{1, 3, 5\}, \{2, 4, 6\}\}$. Both single and every-step participation are special cases of \multiepoch-participation, and as discussed in \citet{choquette22multiepoch}, this setting faithfully captures standard multi-epoch ML training setups.

\paragraph{Banded matrices}
We say a (general) matrix $\bfX$ is $\bands$-banded if for all $i,j \in [n]$, $|i -j| \ge \bands$ implies $\bfX\idx{i}{j} = 0$. While this is off-by-one from the typical definition of bandwidth ($\bfX$ has bandwidth $b-1$), our definition will be useful as it will be natural to match $\bands$-banded matrices with $\minsep$-min-separation. Further, for $\bands$-banded lower-triangular matrices (which will play a central role), $\bands$ intuitively gives the number of bands in the matrix.  

%\btodo{A notation issue: In our code (e.g., \texttt{sensitivity.py}, in some places we use $k$ to denote the number of bands below the main diagonal (following the use of $k$ in numpy and e.g. \url{https://en.wikipedia.org/wiki/Band_matrix}). On the other hand, we claim $k$ is max participation even in the code (and here). Proposal: we keep $k$ for max participation (updating the code). The trickier question (in the code and the paper) is what to do for min-separation and number of bands in the matrix. Strawman Proposal: Use $b$ for both, defining so that in the common case this provides the necessary orthogonality (you want a $b$-banded matrix for $b$-minsep).  This matches how we defined separation in the multi-epoch paper so that every-round participation corresponds to $b=1$. In order to ensure all participations by the same example are orthogonal, this requires a diagonal matrix, which suggests we should define a $(b=1)$-banded matrix to be a diagonal matrix (which, intuitively, also makes sense).  The only place this is awkward is with non-lower-triangular symmetric banded matrices, where it's not clear what $b=2$ would mean. (This is presumably why numpy uses $k$ the way it does). The primary place this will come up for us will be with $X = C^T C$, which when $C$ is lower-triangular banded will be a symmetric banded matrix. But (if this issue actually comes up in the writing), we could perhaps handle this by writing \emph{For lower triangular matrices, $b$-banded means $b$ total bands, including the main diagonal and $b-1$ bands below the main diagonal. We abuse this notation slightly and call a symmetric banded matrix $X$ $b$-banded when it has a total $2b-1$ digaonals, with $b-1$ bands both above and below the main diagonal.}}

\paragraph{The matrix mechanism and sensitivity}
We utilize the matrix mechanism~\citep{Li2015TheMM}, which, provided a factorization $\bfA = \bfB\bfC$, computes the estimate
\begin{equation}\label{eq:mat_mech}
\widehat{\bfA\obs} = \bfB\left(\bfC\obs + \bfz\right),
\end{equation}
where $\bfz$ is a sample from appropriately scaled isotropic Gaussian noise. The scale is determined by the \emph{sensitivity} of the mapping $\obs \mapsto \bfC \obs$. Following \citet{choquette22multiepoch}, let $\bfN$ be the set of all pairs of neighboring streams $\obs$ and $\deltaset := \left\{ \obs - \obsp \mid (\obs, \obsp) \in \bfN \right\}$ represent the set of all possible deltas between neighboring $\obs, \obsp$. We say a $\deltaset$ \textbf{satisfies the participation schema $\Pi$} if the indices of all nonzero elements in each vector $\contrib \in \deltaset$ correspond to some $\pi \in \Pi$ \btodo{May need to make this more precise for scalar vs vector contributions.}. Critically, for linear queries $\deltaset$ fully captures the sensitivity of the query:
\begin{definition}\label{def:sensopmech}
The \textbf{sensitivity} of the matrix factorization mechanism \cref{eq:mat_mech} is defined as
\begin{equation}\label{eq:sensopnorm}
\sensd(\bfC) = \sup_{(\obs, \obsp) \in \bfN} \| \bfC \obs - \bfC \obsp \|_F
 = \sup_{\contrib \in \deltaset} \| \bfC\contrib \|_F. 
\end{equation}
\end{definition}

\begin{prop}[\citet{choquette22multiepoch}]
The sensitivity of $\bfC$ can be upper bounded by.

$$ \max_{\pi \in \Pi} \sum_{ij} | \bfX_{\pi\pi}^{ij} | $$

where $\bfX = \bfC^{\top} \bfC$.  This upper bound is tight when $\bfX \geq 0$.
\end{prop}

\btodo{We probably cannot avoid introducing $\deltaset^1$ and $\deltaset^\mdim$ and the need for the vector-to-scalar reduction. See e.g. \cref{cor:matrix_to_vector_sens}. Probably best to add that background here.}

\ktodo{One of the interesting observations of thinking in the Grothendieck way is: it's not clear that we must frame the problem as scalar-valued, then invoke vector-to-scalar reduction. E.g. we may recover (and even generalize) many of our results from MEMF from just directly analyzing the trace of interest with vector-valued contributions, including those of the nonnegative subsampled $\bfX$ used here. In general, however, framing the problem as scalar-valued then performing the reduction \emph{must} be significantly sharper in some cases, though these cases still require an oracle or good approximation of an $\ell_\infty$ to $\ell_1$ operator norm. I bring this up here because we might be able to simplify some of our presentation by just immediately going for the $d$-dimensional version, explicitly making our $\bfx$ here matrix-valued and viewing the elements of $\pi \in \Pi$ as rows of a matrix, and bypass the need to discuss the reduction.}

\rnote{+1 to putting some of this stuff in the ICML paper, that way we can avoid this nuance here and just cite the relevant sensitivity theorem from that paper.}

Different factorizations $\bfA = \bfB \bfC$ can have very different performance in practice.  Thus, \citet{denisov22matfact} and \citet{choquette22multiepoch} propose optimizing over the space of factorizations, where the objective function is the expected total squared error on $\bfA$, which can be calculated as the product of sensitivity squared (how much noise do we need to add to answer queries in $\bfC$) and the error profile (how much is this noise magnified to go from answers to $\bfC$ to answers to $\bfA$).

\begin{definition}
The \textbf{error profile} of an encoder $\bfC$ is defined as the magnification in error from estimating answers to the queries in $\bfA$ from noisy answers to the queries in $\bfC$.  It can be calculated as $ \norm{\bfA \bfC^{+}}_F^2$, assuming $\bfA$ is in the rowspace of $\bfC$.
\end{definition}

The expected total squared error is invariant to scaling $\bfC$  by a constant, and hence the optimization problem to minimize the error profile under a sensitivity $1$ constraint is given in \cref{prob:optconvex}.
Note that it is useful to express sensitivity and error profile in terms of $\bfX = \bfC^{\top} \bfC$.  The sensitivity can be expressed as $\max_{\contrib \in \deltaset} \bfu \bfX \bfu^{\top} $, and the error profile can be expressed as $\tr{[\bfA^{\top} \bfA \bfX^{+}]}$.  

\begin{problem} \label{prob:optconvex}
The matrix factorization optimization problem requires solving:
\begin{equation} \label{eq:optconvex}
\begin{aligned}
& \underset{\bfX \in \bfS^{n}_{+}}{\text{minimize}}
& & tr[\bfA^{\top} \bfA \bfX^{-1}] \\
& \text{subject to}
& & \max_{\contrib \in \deltaset} \bfu \bfX \bfu^{\top} \leq 1
\end{aligned}
\end{equation}
And choosing $\bfC$ so that $\bfC^{\top} \bfC = \bfX$, e.g., via Cholesky decomposition.
\end{problem}

This is a convex optimization problem, and as such we can find the global minimum with numerical techniques. The formulation of this problem corresponding to \emph{single participation} has been the most-well studied, where the constraint simplifies to $\diag{(\bfX)} \leq \bf1$ \cite{Li2015TheMM,yuan2016convex,mckenna2021hdmm,denisov22matfact}. It is well-understood how to solve this problem in practice, using both primal and dual algorithms.  The generalization to multiple participations with a fixed epoch order has been studied by \citet{choquette22multiepoch}.  %In this paper, our focus will be on a $\Pi_b$ participation schema, which presents some new technical challenges to overcome.

==> cifar10-outline-notes.tex <==

Figure 1.
\begin{itemize}
    \item Mechanisms: opt (20, 100), best banded, DP-SGD
    \item Participation pattern: fixed, shuffled.
    \item Privacy budgets: $[0.1, 2] + [2, 20]$
    \item Metrics: test accuracy.
    \item Hyper-parameters [fixed settings + tuning strategy]:
    \item etc:
\end{itemize}

Ablation on Banded, structure = normalized columns.
\begin{itemize}
    \item Mechanisms: Banded, 
    \item Participation pattern: fixed 
    \item Privacy budgets: $[0.1, 5]$
    \item Metrics: test accuracy, loss. 
    \item Hyper-parameters [fixed settings + tuning strategy]:
    \item etc:
\end{itemize}

Ablation on Stamping (Low Priority)??

